Give and Take: An End-To-End Investigation of Giveaway Scam Conversion Rates

Scams -- fraudulent schemes designed to swindle money from victims -- have existed for as long as recorded history. However, the Internet's combination of low communication cost, global reach, and functional anonymity has allowed scam volumes to reach new heights. Designing effective interventions requires first understanding the context: how scammers reach potential victims, the earnings they make, and any potential bottlenecks for durable interventions. In this short paper, we focus on these questions in the context of cryptocurrency giveaway scams, where victims are tricked into irreversibly transferring funds to scammers under the pretense of even greater returns. Combining data from Twitter, YouTube and Twitch livestreams, landing pages, and cryptocurrency blockchains, we measure how giveaway scams operate at scale. We find that 1 in 1000 scam tweets, and 4 in 100,000 livestream views, net a victim, and that scammers managed to extract nearly \$4.62 million from just hundreds of victims during our measurement window.

==> allowlist.tex <==

\section{Allowlist for Twitter-Based Expansion}
\label{sec:allowlist}

As described in Section~\ref{sec:method-twitter}, we allowed a content template to still be associated with scams if it linked to one of the following 13 top 1M domains: t.me, discord.gg, ripple.com, tinyurl.com, cutt.ly, bit.ly, ow.ly, eep.url, bcns.ai, dlvr.it, twinybots.ch, buff.ly, or ift.tt.

==> partial-pilot-study.tex <==
\section{Pilot Study}
\subsection{Effectiveness of YouTube Search Keywords}
\label{subsec:effectiveness_of_search_keywords}

Based on our pilot analysis, we opted for a set of keywords consisting of the names and ticker symbols of the top 20 cryptocurrencies (as listed on \url{coinmarketcap.com} on July 1, 2023),\footnote{In three cases (for ADA, SOL, and DOT), we appended the word ``coin'' to the ticker symbol to avoid introducing irrelevant streams.} along with two catch-all terms: ``cryptocurrency'' and ``crypto.''  We added other keywords used by the CryptoScamTracker tool~\cite[Table XI]{li2023giveaway} to increase coverage. We found that many of the additional keywords were not useful in expanding our list of relevant streams, and thus stopped expanding our keyword set.

In more detail, we examine the incremental contribution of each search keyword (Table~\ref{tab:search-keywords}) to the set of livestreams returned from the YouTube API. Specifically, we compute the number of YouTube streams (over the 14-day pilot study) that contain search keywords in their metadata (title and description). If one stream contains multiple keywords, we give credit evenly among all keywords.

Figure~\ref{fig:keyword-effectiveness} shows the result. Overall, around 55\% of the streams contained at least one of the search keywords, and the top 20 keywords account for 90\% of those streams. Among the streams that do not contain any search keyword, roughly 50\% are not in English. Sampling English streams that do not contain any keyword, we find that they are either on crypto-adjacent topics (e.g., trading) or completely irrelevant topics (e.g., live street camera).

\subsection{Characteristics of scam livestreams}
\label{subsec:characterisitics_of_scam_streams}
In our 14-day pilot study, we sought to understand the basic characteristics of scam livestreams and websites, which in turn informed the configuration of the parameters in our pipeline (e.g., for how long we record a scam livestream). Specifically, we are interested in two questions: (1) how long a QR code lasts once it appears and (2) how many chat messages are posted during the lifespan of a scam livestream. We started by running our pipeline at maximum capacity on YouTube, with the default setup of recording a stream for two seconds as well as retrieving up to 70 historical chat messages every 7.5 minutes. In addition, for a subset of the livestreams, we kept recording the stream upon detecting a QR code.

With this setup, we manually identified 276 streams that promoted 59 unique giveaway websites. To answer the first question, we examined how long a QR code lasted after we first detected it. For 41 scam livestreams, we continued to record them upon detecting a QR code.
We found that for the majority of the livestreams, a QR code remained displayed continuously for a reasonable amount of time (mean 7,200 seconds and median 3,140 seconds), except for one case where the QR code was displayed periodically for around 15 seconds. This finding suggests that two-second samples are enough to capture a QR code in the livestream, if present. For the latter question, we examined scam streams that had chat messages. We found that all scam streams had few chat messages (less than 10) and no user interactions, and thus decided that 70 historical chat messages every 7.5 minutes is sufficient.

\subsection{Cloaking Behaviors of Scam Websites}
\label{subsec:cloaking_behaviors}
As part of our pilot, we identified four types of cloaking behavior: (1) IP-based cloaking, in which requests from an institutional network resulted in 403 responses but ones from a residential network did not; (2) user agent-based cloaking, in which requests from browsers that were not running on Windows or Mac resulted in 403 responses; (3) customized front pages, in which human interaction was required to click on a button or select a desired cryptocurrency; and (4) anti-bot detection through Cloudflare. As previously mentioned, to counter these behaviors, we (1) used a commercial VPN to mask our IP address; (2) spoofed our User-Agent string to appear as a popular device and browser; (3) added a heuristic module to click through common front pages; and (4) verified our crawler with Cloudflare to avoid triggering their anti-bot detection.
